A Segment-Wise Gaussian Process-Based Ground Segmentation With Local Smoothness Estimation

Both in terrestrial and extraterrestrial environments, the precise and informative model of the ground and the surface ahead is crucial for navigation and obstacle avoidance. The ground surface is not always flat and it may be sloped, bumpy and rough specially in off-road terrestrial scenes. In bumpy and rough scenes the functional relationship of the surface-related features may vary in different areas of the ground, as the structure of the ground surface may vary suddenly and further the measured point cloud of the ground does not bear smoothness. Thus, the ground-related features must be obtained based on local estimates or even point estimates. To tackle this problem, the segment-wise GP-based ground segmentation method with local smoothness estimation is proposed. This method is an extension to our previous method in which a realistic measurement of the length-scale values were provided for the covariance kernel in each line-segment to give precise estimation of the ground for sloped terrains. In this extension, the value of the length-scale is estimated locally for each data point which makes it much more precise for the rough scenes while being not computationally complex and more robust to under-segmentation, sparsity and under-represent-ability. The segment-wise task is performed to estimate a partial continuous model of the ground for each radial range segment. Simulation results show the effectiveness of the proposed method to give a continuous and precise estimation of the ground surface in rough and bumpy scenes while being fast enough for real-world applications.

==> Digest/Latex.tex <==
%%% Note to Authors:
% Please read the following notices carefully before making any modification to the code. Thanks!
% 1) Do NOT change the sort of codes in anyway. For instance, dont move the ''\affiliation'' command above the ''\AddAuthor''.
% 2) There should be NO line breaks or blank lines between codes.
% 3) Do NOT delete the ''%'' sign at the end of lines.
% 4) If authors are all in a same institute, REMOVE the number next to the '\AddAuthor'' command (i.e., ''[1]'') and make sure there is only one ''\affiliation''.
% 5) Please write up to four clauses about your paper using ''\Item'' command. More items will be DELETED.
% 6) Make sure you will change the file name to your submission number. (for example ''315.tex'')
%
\Title{A Gaussian Process-Based Ground Segmentation for Sloped Terrains}%
\AddAuthor[1]{Pouria}{Mehrabi}%
\AddAuthor[1]{Hamid D.}{Taghirad}%
\affiliation[1]{Advanced Robotics and Automated Systems (ARAS) Lab.\\
Faculty of Electrical Engineering, K. N. Toosi University of Technology, Tehran, Iran}%
\Targets{
\Item{This study investigates a method to improve the results of ground segmentation task for driver--less cars using Gaussian process regression in the sloped terrains.}%
\Item{two-dimensional line fitting algorithm is shown to be effective while used as the core of the line extraction algorithm to give better perception of the ground points in sloped areas.}%
\Item{This paper proposes an effective scheme for ground segmentation in sloped area. The proposed method is real-time and does not perform further data truncation.}%
\endinput
}




